Copula-based Sensitivity Analysis for Multi-Treatment Causal Inference with Unobserved Confounding

Recent work has focused on the potential and pitfalls of causal identification in observational studies with multiple simultaneous treatments. Building on previous work, we show that even if the conditional distribution of unmeasured confounders given treatments were known exactly, the causal effects would not in general be identifiable, although they may be partially identified. Given these results, we propose a sensitivity analysis method for characterizing the effects of potential unmeasured confounding, tailored to the multiple treatment setting, that can be used to characterize a range of causal effects that are compatible with the observed data. Our method is based on a copula factorization of the joint distribution of outcomes, treatments, and confounders, and can be layered on top of arbitrary observed data models. We propose a practical implementation of this approach making use of the Gaussian copula, and establish conditions under which causal effects can be bounded. We also describe approaches for reasoning about effects, including calibrating sensitivity parameters, quantifying robustness of effect estimates, and selecting models that are most consistent with prior hypotheses.

==> sections/app-compound.tex <==
\section{Appendix Compound}


\begin{example}[Normal Outcome, Conditional Normal Confounder (with Covariates)]
\begin{align}
U \mid T = 0 &\sim N(0, \tau_0^2)\\
U \mid T = 1 &\sim N(\phi, \tau_1^2)\\
Y(t) \mid U, X &\sim N(\mu_{Xt} + \gamma U, \sigma^2) \\
Y(0) \mid T=0, X &\sim N(\mu_{X0} , \gamma^2\tau_0^2 + \sigma^2) \label{eqn:obs_control}\\
Y(1) \mid T=1, X &\sim N(\mu_{X1} + \gamma\phi, \gamma^2\tau_1^2 + \sigma^2)\label{eqn:obs_treat}
\end{align}

The CATE is $\mu_{X1} - \mu_{X0}$ which is identified conditional on $\gamma\phi$.  Note that 

\begin{align}
\frac{P(T=1 \mid U)}{P(T=0 \mid U)} = \frac{\pi_T}{(1-\pi_T)}\exp\left(-(\frac{1}{2\tau_1^2} - \frac{1}{2\tau_0^2})U^2 - \frac{\phi}{\tau_1^2}U\right)
\label{eqn:normal_treat}
\end{align}

Thus, $T|U$ is logistic in U and $U^2$ (quadratic discriminant analysis).  

Importantly, $\mu_{X0}$, $\gamma^2\tau_0^2 + \sigma^2$, $\mu_{X1} + \gamma\phi$, and $\gamma^2\tau_1^2 + \sigma^2$ are identified.   We want to consider sensitivity parameterizations that leave these quantities unchanged.  Let's consider an important special case with  $\tau_0 = \tau_1 = 1$:

\begin{align}
U \mid T = 0 &\sim N(0, 1)\\
U \mid T = 1 &\sim N(\phi, 1)\\
Y(0) \mid T=0, X &\sim N(\mu_{X0} , \gamma^2 + \sigma^2) \\
Y(1) \mid T=1, X &\sim N(\mu_{X1} + \gamma\phi, \gamma^2 + \sigma^2)\\
\frac{P(T=1 \mid U)}{P(T=0 \mid U)} &= \frac{\pi_T}{(1-\pi_T)}\exp\left(- \phi U\right)
\end{align}

We can calibrate $\gamma$ using the $R^2$ for $U$ in the observed data potential outcome ("how much of the observed data residual variance is explained by the confounder?").  We can calibrate $\phi$ through by considering the coefficients in the T logistic regression or an implicit $R^2$. Note that $|\gamma|$ must be less than or equal to the observed data standard deviations which are identified.  $|\gamma|$ equals the observed data standard deviation when $\sigma^2=0$, i.e. the confounder explains all residual variance.

Interestingly, for any sets of sensitivity parameters $(\gamma_1,\phi_1)$ and $(\gamma_2, \phi_2)$ with $\gamma_1 \phi_1 = \gamma_2\phi_2$ the missing potential outcome distributions are identical. This highlights that we can achieve the same fixed level of confounding by either 1) making the imbalance very large, but the regression coefficient small or 2) making the imbalance very small but the coefficient, $\gamma$ very large. 

\end{example}

%\begin{example}[Normal Outcome, Complete Normal Confounder (with Covariates)]
%\end{example}


\begin{example}[Negative Binomial Regression]

Possible application example: transportation models
% Bayesian Poisson hierarchical models for crash data analysis: Investigating the impact of model choice on site-specific predictions
% \begin{itemize}
% \item \url{https://www.sciencedirect.com/science/article/pii/S0001457507001996}
%     \item \url{https://pdfs.semanticscholar.org/c24a/a81e1d6820b18b2292412b2fb2ae03a66487.pdf}
%     \item \url{https://www.sciencedirect.com/science/article/pii/S0001457511001357}
%     \item \url{https://arxiv.org/pdf/1607.03775.pdf}
%     \item \url{https://www.sciencedirect.com/science/article/pii/S0001457599000500}
%     \item \url{https://www.jstor.org/stable/23024858?seq=1#metadata_info_tab_contents}
% \end{itemize}


\begin{align}
Y(t) \mid \lambda_t &\sim Pois(\lambda_t)\\
\log(\lambda_t) &= a_t + \beta X + \log(G_t) \label{eqn:lambda_spec}\\
(G_t \mid T=t) &= U_t + E_t\\
(G_t \mid T=1\-t) &= U_{1-t} + E_t\\
U_t &\sim \text{Gamma}(\alpha_t, 1)\\
E_t &\sim \text{Gamma}(g_t, 1)
\end{align}

$U_t$ is shared variation due to unobserved confounders, $E_t$ is unshared variation (i.e. treatment effect variation)

This implies
\begin{align}
Y(t) \mid T=t &\sim NegBin\left(\alpha_t + g_t, \frac{\exp(-a_t - \beta X)}{\exp(-a_t - \beta X) + 1}\right)\\
Y(t) \mid T=1\-t &\sim NegBin\left(\alpha_{1-t} + g_t, \frac{\exp(-a_t - \beta X)}{\exp(-a_t - \beta X) + 1}\right)\\
\end{align}

$p_t = \frac{\exp(-a_t - \beta X)}{\exp(-a_t - \beta X) + 1}$ and $r_t = \alpha_t + g_t$ are identified in the observed data.  $\alpha_t \in [0, r_t]$ are sensitivity parameters.  I also wonder if $a_t$ (intercept / treatment effect in \ref{eqn:lambda_spec}) could be decomposed additively to create another sensitivity parameterization?

The discriminant analysis derivations for $U_t$ lead to some further insights.  Writing $U_t$ in EF form, we can easily show that $T \mid U$ is logistic in $\ln(U)$, the sufficient statistic for the Gamma distribution:

\begin{align}
\frac{P(T=1 \mid U)}{P(T=0 \mid U)} = \frac{\pi_T}{(1-\pi_T)}\exp((\alpha_1 - \alpha_0)\ln(U))
\label{eqn:normal_treat}
\end{align}

So a regression of T on $\ln(U)$ determines $\alpha_1 - \alpha_0 \in [-r_t, r_{1\-t}]$.  Notably, this is a one-parameter sensitivity model.

\end{example}

\begin{example}[Binary Outcome with Covariates]
Consider a latent confounder model with binary outcomes.
We posit the existence of a normally distributed latent confounder:
%
\begin{align}
U &\sim N(0, 1)\\
%\pi_t &= \Phi \left( \frac{\psi_T}{ \sqrt{1+\psi_T^2} } \right)\\
%f(U \mid T=1) &\propto \phi(U)\Phi(\psi_T + \psi_T U)\\
%\pi_{Y(t)_{\text{obs}}} &= E[g(\beta_t + \psi_Y U) \mid T = t]
T \mid U, X &\sim \Bern(g(\beta X + \psi_T U))\\
Y(t) \mid U, X &\sim \Bern(\mu_{Yt}(X, U))\label{eqn:normalU binary outcome}\\
\mu_{Yt}(X, U) &= g(\alpha X + \psi_Y U)
\end{align}

Here, the observed outcome distribution is Bernoulli, and characterized by the function
$$
\mu_{Y^{obs}}(X, t) = E[Y(t) \mid T = t, X] = \int_{\mathcal U} \mu_{Yt} f(U \mid T=t, X) dU.
$$

\noindent
%where $f_u(U \mid T)$ is known as the extended skew normal distribution \citep{azzalini2005skew}.
%Again, $\pi_t$ is a continuous monotonic function of $\psi_T$ for any fixed $\alpha$.
%$\alpha$ is not identified from the observed data, but for $\alpha$ fixed to any value, $\psi_T$ is identified.
%Similarly we can use equation \ref{eqn:obs_distribution} to argue that $\pi_{Y(t)_{\text{obs}}}$ is monotonic in $\beta_t$, $\psi_Y$ is completely unidentified and that $\beta_t$ is identified given $\psi_Y$.
In this example, $\mathcal C$ is a smaller family than $\mathcal M$.
In particular, the family $\mathcal C$ only contains distributions whose mean function $\mu_{Yt}$ is monotone in $X$, given the linear dependence in $\mu_{Yt}$ and the monotonicity of $g$.
Meanwhile, the family $\mathcal M$ contains distributions whose mean function $\mu_{Y^{obs}}(X, t)$ can be non-monotone in $X$ because of the indirect dependence on $X$ introduced by the mixing measure $f(U \mid T=t, X)$.
This non-monotonicity is particularly pronounced when $\psi_T$ and $\psi_{Yt}$ have opposite sign for at least one of $t \in \{0, 1\}$.
%
We demonstrate how the posterior predictive distribution of observed data varies as a function of the sensitivity parameters in this model in Figure~\ref{fig:misfit}.
\citet[][Chapter 7]{gustafson2015bayesian} discusses more general versions of this example, noting that there is no general strategy for separating information about parameters $(\alpha, \beta)$ and the sensitivity parameters $\psi$ in a transparent way.
\end{example}

\franks{removed beta-binomial example}
% \begin{example}[Beta Binomial Regression]
% \citep{najera18}

==> sections/r1-sec-latent-confounder.tex <==
\section{Sensitivity Analysis via Copula Parameterizations}
\label{sec:gaussian_copula}

We now establish a sensitivity parameterization for multiple treatment causal inference in a more general class of models by leveraging the copula parameterization in Equation \ref{eqn:fac_y|do(t)}.   For this class of models, we propose an algorithm for estimating any marginal contrast estimand.  \ed{We start with the following general structural equation model}
%
\begin{align}
    U &= \epsilon_u\label{eqn:general_u}\\
    T &= h_{\psi_{T}}(U, \epsilon_t)\\
     \tilde Y &= g_{\psi_Y}(T, U, \epsilon_y) \label{eqn:ytilde_x,u}\\
     Y &= F^{-1}_{Y|t}(F_{\tilde Y \mid T}(\tilde Y ))\label{eqn:y_ytilde_relationship}
\end{align}

\noindent \ed{where $F_{Y \mid T}^{-1}$ is the inverse-CDF of the conditional distribution of $Y$ given $T=t$ and $h_{\psi_T}$ and $g_{\psi_Y}$ are arbitrary functions. In general, neither $h_{\psi_T}$ nor $g_{\psi_Y}$ are identifiable when $U$ is not observed without additional assumptions.}

As illustrated in the previous Section, when $T$ is multivariate, we might gain information about $\psi_T$ if we are willing to make assumptions about the class of latent variable models linking the unmeasured confounders to the treatment.  

\begin{assumption}[Latent variable model identification]
\label{asm:latent_identification}
The potential confounders are continuous and their distribution given treatments, $f\psi_{T}(u \mid t)$, is identifiable up to rotation and scale.
\end{assumption}

\noindent \ed{In this work, we focus on continuous confounders and leave explorations of discrete latent variable models for future work.  Factor model identification is essential for the validity of our sensitivity analysis and will not hold in all settings.  However, while a complete discussion of identifiability in latent variable models is outside the scope of this work, there is a broad range of mathematical settings in which this assumption does hold.  In the previous Section, we noted the classical result due to \citet{anderson1956statistical} establishing identifiablity conditions for linear factor models. \citet{allman2009identifiability} establish identifiability for many latent class models, including those with limited direct dependence between observations; and \citet{miao2020identifying} where weak sufficient conditions are given for similar identifiability in linear models. \citet{barber2022half} consider a set of criterion for establishing when latent variable and \citet{rohe2022vintage} consider identifiability in a broader class of (non-Gaussian) factor models. It is up to the practitioner to decide whether latent variable identifying assumptions are compatible with their applied setting. Finally, in Appendix \ref{sec:causal_equiv} we formalize the idea that it is sufficient to identify the latent variable density only up to invertible linear transformations (rotation and scale). To do so we introduce the notion of a ``causal equivalence class'', which establishes that the substantive causal conclusions do not depend on a particular rotation or scale for the latent confounders.}



\ed{Given $f(y\mid t)$ (identifiable), $f_{\psi_T}(u\mid t)$ (identifiable by Assumption \ref{asm:latent_identification}) and $c_{\psi_Y}$ (nonidentifiable, governed by chosen sensitivity parameter $\psi_Y$)}, we can compute the expected value of any function of the outcome under the intervention distribution, $E[v(Y) \mid do(t)] = \int v(y) f(y \mid do(t)) dy$.   This can be in turn used to compute any marginal contrast estimand. Applying Equation \ref{eqn:fac_y|do(t)}, we write this intervention expectation as
\begin{equation}
\label{eqn:interven_expect}
    E[v(Y) \mid do(t)]\ =  \int v(y) w_\psi(y, t) f(y \mid t) dy,
\end{equation}
where  $w_\psi(y, t) = \int c_{\psi_Y}(F_{Y|t}(y), F^{\psi_T}_{U|t}(u) \mid t) f_{\psi_T}(u) du$ is the importance weight associated with sampling from the observed data distribution instead of the intervention distribution. In practice, we can approximate the marginal distribution of the unobserved confounder with the mixture density $f_{\psi_T}(u) \approx \frac{1}{n} \sum_i f^{\psi_T}(u \mid t_i)$ where $t_i \in  \mathcal{T}$ is the $i$th observed treatment and $\mathcal{T}$ is the set of all observed treatment vectors.  Thus, the importance weight can be approximated as
%
\begin{equation}
\label{eqn:weight}
    w_\psi(y, t) \approx \frac{1}{|\mathcal{T}|}\sum_{t_i \in \mathcal{T}} \left[ \int c_{\psi_Y}(F_{Y|t}(y), F^{\psi_T}_{U|t}(u) \mid t) f_{\psi_T}(u \mid t_i) du\right].
\end{equation}
We use this approximation to derive importance sampling algorithm for computing the expected value in Equation \ref{eqn:interven_expect} for any copula and conditional confounder distributions $f(u \mid t)$ (Appendix A, Algorithm \ref{algm:general}).  This can in turn be used to compute any marginal contrast estimand, $\tau(E[v(y)|do(t_1)], E[v(y)|do(t_2)])$.  








% We also note that we refer to $U$ as \emph{potential} confounders, since the projections of $U$ which are confounding depends on relationship between $Y$ and $U$ as determined by $\Psi_Y$.  




\subsection{The Gaussian Copula Sensitivity Parameterization}

% In Algorithm \ref{algm:general} in Appendix A we describe implementation strategies under more general copulas, and Figure \ref{fig:cop_misspec} in Appendix C we include a simulation study exploring how effects change for non-Gaussian copulas.

\ed{In order to bridge the gap between the interpretable sensitivity parameterization and established theory in the linear Gaussian model (Section \ref{sec:gaussian}) and the more general formulation \ref{eqn:general_u}-\ref{eqn:y_ytilde_relationship}, we provide additional bounds on the omitted variable bias when the copula in \ref{eqn:cop_full} is a Gaussian copula.  } The Gaussian copula is a natural choice when the conditional mean of the outcome is plausibly monotone in the conditional means of the confounders. It includes the special limiting case in which the outcome is comonotone (perfect positive dependence) or countermonotone (perfect negative dependence) with confounders. Outcome-confounder monotonocity is often plausible, at least approximately, conditional on each level $T=t$. 

\begin{assumption}[Gaussian copula]
\label{asm:copula}
The conditional copula between the outcome and $m$-dimensional latent confounders given treatments, is a Gaussian copula.
\end{assumption}

\noindent Then, under Assumptions \ref{asm:latent_identification} and \ref{asm:copula}, we can assume without loss of generality
\begin{equation}
\label{eqn:condition_u}
f(u \mid t) \sim N(\mu_{u|t}, \Sigma_{u\mid t})
\end{equation}
where $\mu_{u\mid t}$ and $\Sigma_{u\mid t}$ can be identified (up to rotation) from a latent variable model on the treatments. We can further rewrite Equations \ref{eqn:ytilde_x,u} - \ref{eqn:y_ytilde_relationship} as 
%
\begin{align}
    \tilde Y &= \gamma_t'U + \epsilon_{\tilde Y} \label{eqn:ytilde_x,u_gauss}\\
     Y &= F^{-1}_{Y|T}(\Phi(\tilde Y -\gamma_t'\mu_{u\mid t}))\label{eqn:y_ytilde_relationship_gauss}
\end{align}
so that $\psi_Y = \{\gamma_t\}$ and $\epsilon_{\tilde Y} \sim N(0, 1 - \gamma_t'\Sigma_{u\mid t}\gamma_t)$ is chosen so that without loss of generality $\text{Var}(\tilde Y \mid T)=1$. 
%

% Identifiability of the latent variable distribution holds for the linear model and may hold approximately for other latent variable models, e.g. variational autoencoders, (VAE) \citep{}. 

The Gaussian copula under this model is fully determined by the covariance matrix
\begin{equation} 
\label{eqn:gaussian_copula}
    \text{Cov}([\tilde{Y}, U] \mid T=t) = 
    \begin{bmatrix}
        1 & \gamma_t'\Sigma_{u|t}\\
    \ \Sigma_{u|t}\gamma_t & \ \Sigma_{u|t}
    \end{bmatrix}
\end{equation}
with parameters $\psi_T = \{\mu_{u\mid t}, \Sigma_{u\mid t} : t \in \mathcal{T}\}$ and $\psi_Y = \{\gamma_t : \mathcal{T}\}$ where $\mathcal{T}$ is the space of all treatments.  Given Assumption \ref{asm:latent_identification}, $\psi_Y = \{\gamma_t\}$ is the sole $m-$dimensional sensitivity vector governing the magnitude of the omitted variable bias. Per Assumption \ref{asm:latent_identification}, we assume that $\psi_T$ is identified up to invertible linear transformations of $U$, and explore the range of possible causal effects for different $\gamma_t$ satisfying $\gamma'_t\Sigma_{u \mid t}\gamma_t \leq 1$.  


In Algorithm \ref{algm:gaussian} (Appendix A), we provide a modification of Algorithm \ref{algm:general} tailored to the Gaussian copula setting.  At a high level, we compute a Monte Carlo estimate of $f(y \mid do(t))$ via the following three step procedure: (1) draw a sample from $f(u)$, (2)  compute the conditional density of the Gaussianized outcome $f(\tilde y \mid u, t)$ via the Gaussian copula and (3) transform $\tilde y$ back to original space via the conditional quantile function $F^{-1}_{Y\mid t}$ (see Figure \ref{fig:calibration}, Appendix A). In the following Sections, we introduce some theoretical insights about our approach and provide a method for calibrating the magnitude of $\gamma_t$ and reasoning about its direction. 






% For our sensitivity analysis, we emphasize the importance of two criteria: 1) the observed data fit should be invariant to all  sensitivity parameters (no observable implications) and 2) the sensitivity analysis should be widely applicable to a range of models, e.g. for both continuous and discrete data. In order to satisfy these criteria, 


% The factorization proposed here is particularly useful since $f(y \mid t)$ and (potentially) $f(u \mid t)$ are identifiable and distinct from the unidentifiable copula.  This factorization ensures that the settings for the $\psi_Y$ has no effect on the densities of the observables. 

% \label{sec:generalization}




